Scalable Bayesian Non-Negative Tensor Factorization for Massive Count Data

We present a Bayesian non-negative tensor factorization model for count-valued tensor data, and develop scalable inference algorithms (both batch and online) for dealing with massive tensors. Our generative model can handle overdispersed counts as well as infer the rank of the decomposition. Moreover, leveraging a reparameterization of the Poisson distribution as a multinomial facilitates conjugacy in the model and enables simple and efficient Gibbs sampling and variational Bayes (VB) inference updates, with a computational cost that only depends on the number of nonzeros in the tensor. The model also provides a nice interpretability for the factors; in our model, each factor corresponds to a "topic". We develop a set of online inference algorithms that allow further scaling up the model to massive tensors, for which batch inference methods may be infeasible. We apply our framework on diverse real-world applications, such as \emph{multiway} topic modeling on a scientific publications database, analyzing a political science data set, and analyzing a massive household transactions data set.

==> macros.tex <==
  \newcommand{\initial}  {
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Macro initial declares variables and initializes the       %
   % variables and the unitlength.  Macro reinit resets the     %
   % values of the variables and the unitlength to the          %
   % original values.                                           %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %
     \setlength{\unitlength}{.1pt}
     \newcount\xi        \newcount\yi
     \xi=0               \yi=300
     % coordinates of lower left corner
     \newcount\pht       \pht=900            % picture height
     \newcount\pw        \pw=400             % picture width
     \newcount\xbox      \xbox=50            % width of minipage
     \newcount\len  }    % general purpose variable     
     % end macro initial
  \newcommand{\reinit}   {\xi=0   \yi=300    \xbox=50  
              \setlength{\unitlength}{.1pt}
              \pht=900 \pw=400  }   % end macro reinit
 \newcommand{\cbranch}[9]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The cbranch macro draws vertical branches as single and    %
  % double bonds, up and down.                                 %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \begin{picture}(\pw,\pht)(-\xi,-\yi)
               \put(0,200)    {#1}                 % upper subst.
   \ifx#2S     \put(40,85)    {\line(0,1)  {100}}  % single up
   \else\ifx#2D\multiput(27,85)(26,0){2}           % double up   
                              {\line(0,1)  {100}} \fi \fi
   \ifx#4Q     \put(-305,0)   {\makebox(300,87)[r]{#3}}
                              % left substituent without bond 
   \else       \put(-455,0)   {\makebox(300,87)[r]{#3}} \fi
                              % left substituent with bond
   \ifx#4S     \put(-150,33)  {\line(1,0)  {140}}  % single left
   \else\ifx#4D\multiput(-150,20)(0,26){2}         % double left
                              {\line(1,0)  {140}} \fi \fi
               \put(0,0)      {#5}                 % center 
                                                   %  atom(s)
   \ifx#6S     \put(90,33)    {\line(1,0)  {140}}  % single right
   \else\ifx#6D\multiput(90,20)(0,26){2}           % double right
                              {\line(1,0)  {140}} \fi \fi
               \put(240,0)    {#7}                 % right subst.
   \ifx#8S     \put(40,-15)   {\line(0,-1) {100}}  % single down
   \else\ifx#8D\multiput(27,-15)(26,0){2}          % double down
                              {\line(0,-1) {100}} \fi \fi
               \put(0,-210)   {#9}                 % lower subst.
  \end{picture}           }   % end cbranch macro
 \newcommand{\tbranch}[7]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Macro tbranch draws structures with vertical branches,     %
  % single or double bonds, going up or down.                  %
  % This macro uses the LaTeX tabbing mechanism.               %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \begin{minipage}{\xbox pt}
   \begin{tabbing}
    $#3$\= $#4$\+ \kill
           $#1$   \\ [-#7pt]     % print top subst.
    \ifx#2S                      % vertical bond going up
           \hspace{4pt}\rule{0.4pt}{8pt}  \\ [-#7pt]\fi
    \ifx#2D
           \hspace{2pt}\rule{0.4pt}{8pt}  
           \hspace{-2pt}\rule{0.4pt}{8pt} \\ [-#7pt]\fi
           \- \kill
    $#3$\> $#4$\+ \\ [-#7pt]     % substituents on print line
    \ifx#5S                      % vertical bond going down
           \hspace{4pt}\rule{0.4pt}{8pt}  \\ [-#7pt]\fi
    \ifx#5D
           \hspace{2pt}\rule{0.4pt}{8pt}    
           \hspace{-2pt}\rule{0.4pt}{8pt} \\ [-#7pt]\fi
           $#6$
  \end{tabbing}
 \end{minipage}    }             % end tbranch macro
 \newcommand{\ethene}[4]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a horizontal ethene fragment with    %
  % four variable substituents.                              %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(-405,170)  {\makebox(300,87)[r]{#1}}       % upper left
                                                    %  subst.  
    \put(-405,-185) {\makebox(300,87)[r]{#3}}       % lower left
                                                    %  subst.
    \put(0,70)      {\line(-1,1)        {100}}      % NW bond
    \put(0,0)       {\line(-1,-1)       {100}}      % SW bond
    \put(0,0)       {C}                             % left C
    \multiput(90,20)(0,25){2} {\line(1,0){140}}     % double bond
    \put(240,0)     {C}                             % right C
    \put(315,70)    {\line(1,1)         {100}}      % NE bond
    \put(315,0)     {\line(1,-1)        {100}}      % SE bond
    \put(425,170)   {#2}                            % upper right
                                                    %  subst.
    \put(425,-170)  {#4}                            % lower right
                                                    %  subst.
   \end{picture}               }              % end ethene macro
 \newcommand{\upethene}[4]   {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a vertical ethene fragment with four   %
  % variable substituents.                                     %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(-430,360)           {\makebox(300,87)[r]{#1}} % NW subst.
    \put(-430,-150)          {\makebox(300,87)[r]{#2}} % SW subst.
    \put(210,370)            {#3}                      % NE subst.
    \put(210,-140)           {#4}                      % SE subst.
    \put(0,300)              {\line(-5,3)  {121}}      % NW bond
    \put(0,230)              {C}                       % upper C
    \put(20,80)              {\line(0,1)   {140}}      % vertical
    \put(46,80)              {\line(0,1)   {140}}      %  d. bond
    \put(0,0)                {C}                       % lower C
    \put(0,0)                {\line(-5,-3) {121}}      % SW bond
    \put(80,300)             {\line(5,3)   {121}}      % NE bond
    \put(80,0)               {\line(5,-3)  {121}}      % SE bond
   \end{picture}             }              % end upethene macro            
 \newcommand{\cright}[7]        {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a trigonal fragment, opening to the     %
  % right. The fragment has a variable center atom and three    %
  % variable substituents. Bonds can be single or double.       %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \ifx#2Q \put(-305,-15){\makebox(300,87)[r]{#1}}   % left sub.
     \else  \put(-455,-15){\makebox(300,87)[r]{#1}} \fi
    \ifx#2S \put(-150,33)    {\line(1,0)   {140}} \fi % single 
                                                      % hor. bond
    \ifx#2D \put(-150,20)    {\line(1,0)   {140}}     % hor.
            \put(-150,46)    {\line(1,0)   {140}} \fi %  d. bond
    \put(0,0)                {#3}                     % center
                                                      %  atoms
    \ifx#4S \put(80,70)      {\line(1,1)   {100}} \fi % NE single
                                                      %  bond
    \ifx#4D \put(71,79)      {\line(1,1)   {100}}
            \put(89,61)      {\line(1,1)   {100}} \fi % NE double
    \put(185,170)            {#5}                     % NE subst.
    \ifx#6S \put(80,0)       {\line(1,-1)  {100}} \fi % SE single
    \ifx#6D \put(71,-9)      {\line(1,-1)  {100}}     % SE double
            \put(89,9)       {\line(1,-1)  {100}} \fi %  bond
    \put(185,-170)           {#7}                     % SE subst.
   \end{picture}             }               % end cright macro
 \newcommand{\cleft}[7]      {
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % This macro typesets a trigonal fragment, opening to the     %
 % left. The fragment has a variable center atom and three     %
 % variable substituents. Bonds can be single or double.       %
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % 
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(-405,160)           {\makebox(300,87)[r]{#1}} % NW subst.
    \ifx#2S \put(0,70)       {\line(-1,1)  {100}} \fi  % NW single
                                                       %  bond
    \ifx#2D \put(9,79)       {\line(-1,1)  {100}}      % NW double
            \put(-9,61)      {\line(-1,1)  {100}} \fi  %  bond
    \put(0,0)                {#3}                      % center 
                                                       %  atoms(s)
    \ifx#4S \put(0,0)        {\line(-1,-1) {100}} \fi  % SW single
    \ifx#4D \put(-9,9)       {\line(-1,-1) {100}}      % SW double
            \put(9,-9)       {\line(-1,-1) {100}} \fi  %  bond
    \put(-405,-185)          {\makebox(300,87)[r]{#5}} % SW subst.
    \ifx#6S \put(90,33)      {\line(1,0)   {140}} \fi  % hor.
                                                       %  single
    \ifx#6D \put(90,20)      {\line(1,0)   {140}}      %  double
            \put(90,46)      {\line(1,0)   {140}} \fi  %  bond
    \put(240,0)              {#7}                      % right sub.
   \end{picture}             }               % end cleft macro
 \newcommand{\chemup}[7]        {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a trigonal fragment, opening          %
  % upwards.  The fragment has a variable center atom and     %
  % three variable substituents.  Bonds are single or         %
  % double.                                                   %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(-430,130)           {\makebox(300,87)[r]{#1}} % NW subst.
    \ifx#2S \put(0,70)       {\line(-5,3)  {121}} \fi  % NW single
    \ifx#2D \put(7,81)       {\line(-5,3)  {121}}      % NW double
            \put(-7,59)      {\line(-5,3)  {121}} \fi  %    bond
    \put(0,0)                {#3}                      % center 
                                                       %  atom(s)
    \ifx#4S \put(33,-10)     {\line(0,-1)  {140}} \fi  % vertical 
                                                       %  single
    \ifx#4D \put(20,-10)     {\line(0,-1)  {140}}      % vertical
            \put(46,-10)     {\line(0,-1)  {140}} \fi  %  double
    \put(0,-230)             {#5}                      % bottom
                                                       %  subst.
    \ifx#6S \put(80,70)      {\line(5,3)   {121}} \fi  % NE single
    \ifx#6D \put(73,81)      {\line(5,3)   {121}}      % NE double
            \put(87,59)      {\line(5,3)   {121}} \fi  %    bond
    \put(210,140)            {#7}                      % NE subst.
  \end{picture}              }                % end chemup macro
 \newcommand{\cdown}[7]      {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a trigonal fragment, opening            %
  % downwards. The fragment has a variable center atom and      %
  % three variable substituents. Bonds are single or double.    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(0,230)              {#1}                      % upper sub.
    \ifx#2S \put(33,80)      {\line(0,1)   {140}} \fi  % vert. 
                                                       %  single
    \ifx#2D \put(20,80)      {\line(0,1)   {140}}      %  double
            \put(46,80)      {\line(0,1)   {140}} \fi
    \put(0,0)                {#3}                      % center 
                                                       %  atom(s)
    \ifx#4S \put(0,0)        {\line(-5,-3) {121}} \fi  % SW single
    \ifx#4D \put(-7,11)      {\line(-5,-3) {121}}      % SW double
            \put(7,-11)      {\line(-5,-3) {121}} \fi  %    bond
    \put(-430,-150)          {\makebox(300,87)[r]{#5}} % SW subst.
    \ifx#6S \put(80,0)       {\line(5,-3)  {121}} \fi  % SE bond
    \ifx#6D \put(87,11)      {\line(5,-3)  {121}}      % SE double
            \put(73,-11)     {\line(5,-3)  {121}} \fi  %    bond
    \put(210,-140)           {#7}                      % SE subst.
   \end{picture}             }               % end cdown macro
 \newcommand{\csquare}[5]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a fragment that consists of a variable  %
  % center atom with four variable substituents pointing to     %
  % the four corners of a square.                               %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(-405,160)           {\makebox(300,87)[r]{#1}} % NW subst.
    \put(0,70)               {\line(-1,1)  {100}}      % NW bond
    \put(0,0)                {#3}                      % center 
                                                       %  atom
    \put(0,0)                {\line(-1,-1) {100}}      % SW bond 
    \put(-405,-185)          {\makebox(300,87)[r]{#4}} % SW subst.
    \put(80,70)              {\line(1,1)   {100}}      % NE bond
    \put(185,170)            {#2}                      % NE subst.
    \put(80,0)               {\line(1,-1)  {100}}      % SE bond
    \put(185,-170)           {#5}                      % SE subst.
  \end{picture}              }                % end csquare macro       
 \newcommand{\ccirc}[4]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The ccirc macro draws a circle with 2 substituents          %
  % infront of the circle and 2 behind it to give a             %
  % threedimensional impression.                                %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
 \begin{picture}(\pw,\pht)(-\xi,-\yi)
   \put(90,0)    {\circle{180}}
   \put(90,90)   {\line(0,1)   {70}}        % behind and up
   \put(60,170)  {#1}
   \thicklines
   \put(30,10)   {\line(-5,2)  {140}}       % in front
   \put(-415,30) {\makebox(300,87)[r]{#2}}  %  and left
   \put(150,10)  {\line(5,2)   {140}}       % in front 
   \put(300,30)  {#3}                       %  and right
   \thinlines
   \put(90,-90)  {\line(0,-1) {90}}         % behind and
   \put(60,-260) {#4}                       %  down
 \end{picture}     }                % end ccirc macro

 \newcommand{\threering}[9]     {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The threering macro typesets the cyclopropane ring       %
  % with optional substituents, an optional double bond,     %
  % and a plus inside the ring for aromaticity.              %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
       \put(300,0)     {\line(-3,-5) {150}}     % bond 1 to 2
       \put(150,-244)  {\line(-3,5)  {150}}     % bond 2 to 3
       \put(0,0)       {\line(1,0)   {300}}     % bond 3 to 1
       \ifx#7D \put(40,-40){\line(1,0){220}}\fi % double 3 to 1
       \ifx#1Q                                  % subst. on 1
         \else\put(300,0)    {\line(5,3)   {128}}
              \put(433,50)   {#1}           \fi
       \ifx#2Q                                  % subst. on 2
         \else\ifx#9C \put(150,-244) {\line(0,-1){100}}
                      \put(114,-424) {#2}  % on straight bond
                 \else\put(150,-244) {\line(5,-3)  {128}}
                      \put(283,-344) {#2} \fi \fi % slanted 
       \ifx#2Q                                  % subst. on 2
         \else\ifx#5Q \put(150,-244) {\line(0,-1){100}}
                      \put(114,-424) {#2}  % on straight bond
                 \else\put(150,-244) {\line(5,-3)  {128}}
                      \put(283,-344) {#2} \fi \fi % slanted 
       \ifx#3Q                                  % subst. on 3
         \else\put(0,0)      {\line(-5,3)  {128}}
              \put(-430,34) {\makebox(300,87)[r]{#3}} \fi
       \ifx#4Q                                  % second subst. 
         \else\put(300,0)    {\line(5,-3)  {128}} %  on 1
              \put(433,-100) {#4}           \fi
       \ifx#5Q                                  % second subst. 
         \else\put(150,-244) {\line(-5,-3) {128}} %  on 2
              \put(-280,-360){\makebox(300,87)[r]{#5}}  \fi
       \ifx#6Q                                  % second subst. 
         \else\put(0,0)      {\line(-5,-3) {128}} %  on 3
              \put(-430,-116){\makebox(300,87)[r]{#6}} \fi
       \ifx#8Q
         \else\multiput(135,-244)(30,0){2}      % outside 
              {\line(0,-1)   {100}}             %  double
              \put(114,-424) {#8}           \fi %  on 2
       \ifx#9C \put(150,-90){\circle{120}}   % circle with +
               \put(110,-120){+}            \fi
       \end{picture}            }   % end cycloprop. macro
 \newcommand{\fourring}[9]      {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The fourring macro typesets the cyclobutane ring with      %
  % optional substituents and double bonds.                    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
      \put(300,300)   {\line(0,-1)  {300}}      % bond 1 to 2
      \put(300,0)     {\line(-1,0)  {300}}      %      2 to 3
      \put(0,0)       {\line(0,1)   {300}}      %      3 to 4
      \put(0,300)     {\line(1,0)   {300}}      %      4 to 1
      \ifx#7D\put(260,260){\line(0,-1){220}}\fi % double 1 to 2
      \ifx#8D\put(40,40)  {\line(0,1) {220}}\fi % double 3 to 4
      \ifx#1Q                                   % subst. on 1
        \else\put(300,300){\line(5,3) {128}}  
             \put(433,350){#1}              \fi
      \ifx#2Q                                   % subst. on 2
        \else\put(300,0)  {\line(5,-3){128}}
             \put(433,-100){#2}             \fi
      \ifx#3Q                                   % subst. on 3
        \else\put(0,0)    {\line(-5,-3){128}}
             \put(-430,-116){\makebox(300,87)[r]{#3}} \fi
      \ifx#4Q                                   % subst. on 4
        \else\put(0,300)  {\line(-5,3) {128}}
             \put(-430,334){\makebox(300,87)[r]{#4}}  \fi
      \ifx#5Q                                   % second subst. 
        \else\put(300,300){\line(5,-3) {128}}   %  on 1
             \put(433,200){#5}              \fi
      \ifx#6Q                                   % second subst. 
        \else\put(0,300)  {\line(-5,-3){128}}   %  on 4
             \put(-430,184){\makebox(300,87)[r]{#6}}  \fi
      \ifx#9Q                                   % outs. double 
        \else\multiput(280,-5)(20,30){2}        %  and subst.
             {\line(1,-1){100}} \put(405,-140){#9}   \fi % on 2
    \end{picture}         }             % end cyclobutane macro
   \newcommand{\fivering}[9]    {
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % This macro typesets the cyclopentane ring with optional    %
    % substituents and double bonds. A minus sign in a circle    %
    % can be put inside the ring to denote aromaticity.          %
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %
       \begin{picture}(\pw,\pht)(-\xi,-\yi)
        \put(342,200)    {\line(0,-1)   {200}}       % bond 1 to 2
        \put(342,0)      {\line(-5,-3)  {171}}       % bond 2 to 3
        \put(171,-103)   {\line(-5,3)   {171}}       % bond 3 to 4
        \put(0,0)        {\line(0,1)    {200}}       % bond 4 to 5
        \put(0,200)      {\line(1,0)    {342}}       % bond 5 to 1
        \ifx#1Q                                      % subst. on 1 
          \else\put(342,200)   {\line(5,3)  {128}}
               \put(475,250)   {#1}              \fi
        \ifx#2Q                                      % subst. on 2
          \else\put(342,0)     {\line(5,-3) {128}}
               \put(475,-100)  {#2}              \fi
        \ifx#3Q                                      % subst. on 3
          \else\put(171,-103)  {\line(0,-1) {100}}
               \put(150,-283)  {#3}              \fi
        \ifx#4Q                                      % subst. on 4
          \else\put(0,0)       {\line(-5,-3){128}}
               \put(-430,-116) {\makebox(300,87)[r]{#4}}  \fi
        \ifx#5Q                                      % subst. on 5
          \else\put(0,200)     {\line(-5,3) {128}}
               \put(-430,234)  {\makebox(300,87)[r]{#5}}  \fi
        \ifx#6D\put(316,174)   {\line(0,-1) {148}}   % double 1,2
          \else\ifx#6S
                 \else\put(342,200) {\line(5,-3) {128}}
                      \put(475,100){#6}   \fi        % second sub.
        \fi                                          %  on 1
        \ifx#7D\put(26,26)     {\line(0,1)  {148}}   % double 4,5
          \else\ifx#7S
                 \else\put(0,200){\line(-5,-3){128}} % second sub. 
                      \put(-430,84){\makebox(300,87)[r]{#7}}  \fi
        \fi                                          %  on 5
        \ifx#8Q                                      % outs. double 
          \else\multiput(156,-103)(30,0){2}          %  and subst. 
               {\line(0,-1) {100}} \put(135,-283){#8}  \fi  % on 3
        \ifx#9C\put(171,60)    {\circle{210}}        % circle and 
               \put(130,35)    {$-$}       \fi       %  minus
      \end{picture}          }                 % end 5-ring macro
  \newcommand{\sixring}[9]   {
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % The sixring macro draws standard carbon sixrings in the    %
   % shape of a regular hexagon. There are optional ring        %
   % double bonds and substituents.                             %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(342,200)  {\line(0,-1)  {200}}          % bond 1 to 2
    \put(342,0)    {\line(-5,-3) {171}}          % bond 2 to 3
    \put(171,-103) {\line(-5,3)  {171}}          % bond 3 to 4
    \put(0,0)      {\line(0,1)   {200}}          % bond 4 to 5      
    \put(0,200)    {\line(5,3)   {171}}          % bond 5 to 6
    \put(171,303)  {\line(5,-3)  {171}}          % bond 6 to 1
    \ifx#7D                                      % d. bond 1,2 
      \put(316,174)   {\line(0,-1)  {148}}       
      \else \ifx#7S                              % 2. sub. on 1
            \else\put(342,200) {\line(5,-3) {128}}
                 \put(475,100) {#7}    \fi  \fi
    \ifx#8D
      \put(162,-67)   {\line(-5,3)  {126}}       % double 3 to 4
      \else\ifx#8S
           \else\put(156,-203) {\line(0,1){100}} % outside 
                                                 %  double and
                \put(186,-203) {\line(0,1){100}} %  subst. on 3
                \put(135,-283) {#8}    \fi  \fi
    \ifx#9D
      \put(36,191)    {\line(5,3)   {126}} \fi   % double 5 to 6   
    \ifx#9C \put(171,100) {\circle{250}}   \fi   % circle for 
                                                 %  aromaticity
    \ifx#1Q                                      % subst. on 1
      \else\put(342,200)  {\line(5,3){128}}
           \put(475,250)  {#1}             \fi
    \ifx#2Q
      \else\put(342,0)    {\line(5,-3){128}}     % subst. on 2
           \put(475,-100)    {#2}          \fi
    \ifx#3Q
      \else\put(171,-203) {\line(0,1){100}}
           \put(150,-283) {#3}             \fi   % subst. on 3
    \ifx#4Q
       \else\put(0,0)     {\line(-5,-3){128}}    % subst. on 4
            \put(-430,-116){\makebox(300,87)[r]{#4}}  \fi
    \ifx#5Q
      \else\put(0,200)    {\line(-5,3){128}}     % subst. on 5
           \put(-430,234) {\makebox(300,87)[r]{#5}}   \fi
    \ifx#6Q
      \else\put(171,303)  {\line(0,1){100}}      % subst. on 6
           \put(150,410)  {#6}             \fi
    \ifx#7D  \ifx#9C \message{Error: ring double bond 
                             simultaneous with circle}
    \fi   \fi
   \end{picture}           }                % end sixring macro
  \newcommand{\sixringa}[9]   {
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % This macro differs from the original sixring macro only    %
   % in the position of the double bonds in the ring.           %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
       \put(342,200)  {\line(0,-1)  {200}}          % bond 1 to 2
       \put(342,0)    {\line(-5,-3) {171}}          % bond 2 to 3
       \put(171,-103) {\line(-5,3)  {171}}          % bond 3 to 4
       \put(0,0)      {\line(0,1)   {200}}          % bond 4 to 5      
       \put(0,200)    {\line(5,3)   {171}}          % bond 5 to 6
       \put(171,303)  {\line(5,-3)  {171}}          % bond 6 to 1
       \ifx#7D                                      % double 1,6 
         \put(306,191)   {\line(-5,3)  {126}}       
         \else \ifx#7S                              % second subst. 
               \else\put(342,200) {\line(5,-3) {128}}
                    \put(475,100) {#7}    \fi  \fi  %  on 1
       \ifx#8D
         \put(178,-67)   {\line(5,3)   {126}}       % double 3,2
         \else\ifx#8S
              \else\put(156,-203) {\line(0,1){100}} % outs. double 
                   \put(186,-203) {\line(0,1){100}} %  and subst. 
                   \put(135,-283) {#8}    \fi   \fi %  on 3
       \ifx#9D
         \put(26,26)     {\line(0,1)   {148}} \fi   % double 4,5   
       \ifx#9C \put(171,100) {\circle{250}}   \fi   % circle for
                                                    %  aromaticity
       \ifx#1Q                                      % subst. on 1
         \else\put(342,200)  {\line(5,3){128}}
              \put(475,250)  {#1}             \fi
       \ifx#2Q
         \else\put(342,0)    {\line(5,-3){128}}     % subst. on 2
              \put(475,-100)    {#2}          \fi
      \ifx#3Q
         \else\put(171,-203) {\line(0,1){100}}
              \put(150,-283) {#3}             \fi   % subst. on 3
       \ifx#4Q
          \else\put(0,0)     {\line(-5,-3){128}}    % subst. on 4
               \put(-430,-116){\makebox(300,87)[r]{#4}} \fi
       \ifx#5Q
         \else\put(0,200)    {\line(-5,3){128}}     % subst. on 5
              \put(-430,234) {\makebox(300,87)[r]{#5}}  \fi
       \ifx#6Q
         \else\put(171,303)  {\line(0,1){100}}      % subst. on 6
              \put(150,410)  {#6}             \fi
       \ifx#7D  \ifx#9C \message{Error: ring double bond with 
                                        circle} \fi   \fi
      \end{picture}           }             % end sixringa macro
  \newcommand{\sixringb}[9]   {
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % This variation of the sixring can typeset all combina-     %
   % tions of double bonds in the ring through argument 9.      %
   % A para-quinoid structure is also possible.                 %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % macros to typeset the ring double bonds:
  \newcommand{\di}   {\put(316,174){\line(0,-1){148}}} %double 1-2
  \newcommand{\dii}  {\put(178,-67){\line(5,3) {126}}} %double 2-3
  \newcommand{\diii} {\put(162,-67){\line(-5,3){126}}} %double 3-4
  \newcommand{\dfour}{\put(26,26)  {\line(0,1) {148}}} %double 4-5
  \newcommand{\dv}   {\put(36,191) {\line(5,3) {126}}} %double 5-6
  \newcommand{\dsix} {\put(306,191){\line(-5,3){126}}} %double 6-1
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
       \put(342,200)  {\line(0,-1)  {200}}          % bond 1 to 2
       \put(342,0)    {\line(-5,-3) {171}}          % bond 2 to 3
       \put(171,-103) {\line(-5,3)  {171}}          % bond 3 to 4
       \put(0,0)      {\line(0,1)   {200}}          % bond 4 to 5      
       \put(0,200)    {\line(5,3)   {171}}          % bond 5 to 6
       \put(171,303)  {\line(5,-3)  {171}}          % bond 6 to 1
       \ifx#7Q                                      
        \else\put(158,303) {\line(0,1) {100}}       % outs. double
             \put(184,303) {\line(0,1) {100}}       %  bond and 
             \put(130,420) {#7}    \fi              %  sub. on 6
       \ifx#8Q
        \else\put(156,-203){\line(0,1){100}}        % outs. double 
             \put(186,-203){\line(0,1){100}}        %  bond and 
             \put(135,-283) {#8}   \fi              %  sub.on 3
       % 17 double bond combinations:
       \ifcase#9 \put(171,100) {\circle{250}}        % circle 
         \or \di \or \dii \or \or diii \or \di \diii % arg 9=1-5       
         \or \or \or dfour \or \dfour \di            % arg 9=6-9
         \or \dfour \dii \or \or \or \or \or \or \dv % arg 9=10-16
         \or \dv \di \or \dv \dii \or \or \dv \diii  % arg 9=17-20
         \or \dv \diii \di \or \or \or \or \or \or   % arg 9=21-27
         \or \or \or \or \or \dsix \or \or \dsix \dii %      28-34
         \or \or \dsix \diii \or \or \or             % arg 9=35-39
         \or \dsix \dfour \or \or \dsix \dfour \dii  % arg 9=40-42
       \fi
       \ifx#1Q                                      % subst. on 1
         \else\put(342,200)  {\line(5,3){128}}
              \put(475,250)  {#1}       \fi
       \ifx#2Q
         \else\put(342,0)    {\line(5,-3){128}}     % subst. on 2
              \put(475,-100)    {#2}    \fi
      \ifx#3Q
         \else\put(171,-203) {\line(0,1){100}}
              \put(150,-283) {#3}       \fi         % subst. on 3
       \ifx#4Q
          \else\put(0,0)     {\line(-5,-3){128}}    % subst. on 4
               \put(-430,-116){\makebox(300,87)[r]{#4}}  \fi
       \ifx#5Q
         \else\put(0,200)    {\line(-5,3){128}}     % subst. on 5
              \put(-430,234) {\makebox(300,87)[r]{#5}}   \fi
       \ifx#6Q
         \else\put(171,303)  {\line(0,1){100}}      % subst. on 6
              \put(150,410)  {#6}       \fi
       \ifx#7D  \ifx#9C \message{Error: ring double bond with
                                        circle}  \fi  \fi
      \end{picture}           }              % end sixringb macro
  \newcommand{\chair}[8]       {
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % The chair macro typesets the saturated carbon sixring in   %
   % its most favorable conformation. Axial and equatorial      %
   % substituents can be attached in 4 positions.               %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
      \put(0,0)       {\line(3,-4)  {170}}      % bond 1 to 2
      \put(170,-226)  {\line(3,1)   {403}}      %      2 to 3
      \put(573,-91)   {\line(6,-1)  {210}}      %      3 to 4
      \put(783,-126)  {\line(-3,4)  {170}}      %      4 to 5
      \put(613,100)   {\line(-3,-1) {403}}      %      5 to 6
      \put(210,-35)   {\line(-6,1)  {210}}      %      6 to 1
                                          % bonds to subst. :
      \put(0,0)       {\line(0,1)   {100}}      % axial on 1
      \put(170,-226)  {\line(0,-1)  {100}}      % axial on 2
      \put(573,-91)   {\line(0,1)   {100}}      % axial on 3
      \put(783,-126)  {\line(0,-1)  {100}}      % axial on 4
      \put(613,100)   {\line(0,1)   {100}}      % axial on 5
      \put(210,-35)   {\line(0,-1)  {100}}      % axial on 6
      \put(0,0)       {\line(-3,-1) {128}}      % eq. on 1
      \put(170,-226)  {\line(-3,1)  {128}}      % eq. on 2
      \put(573,-91)   {\line(3,-1)  {128}}      % eq. on 3
      \put(783,-126)  {\line(3,1)   {128}}      % eq. on 4
      \put(613,100)   {\line(3,-1)  {128}}      % eq. on 5
      \put(210,-35)   {\line(-3,1)  {128}}      % eq on 6
                                          % variable subst.:
      \ifx#1Q\else\put(-30,110)     {#1}    \fi % axial on 1
      \ifx#2Q\else\put(140,-406)    {#2}    \fi % axial on 2
      \ifx#3Q\else\put(543,9)       {#3}    \fi % axial on 3
      \ifx#4Q\else\put(753,-306)    {#4}    \fi % axial on 4
      \ifx#5Q\else\put(-430,-85) {\makebox(300,87)[r]{#5}}
      \fi                                       % eq. on 1
      \ifx#6Q\else\put(-260,-226){\makebox(300,87)[r]{#6}}
      \fi                                       % eq. on 2
      \ifx#7Q\else\put(415,-230) {\makebox(300,87)[r]{#7}}
      \fi                                       % eq. on 3
      \ifx#8Q\else\put(916,-115)    {#8}    \fi % eq. on 4
     \end{picture}              }         % end chair macro
 \newcommand{\naphth}[9]        {       
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets the naphthalene ring system.           %
  % One or both rings can be saturated. An optional sub-       %
  % stituent is possible at each ring position.                %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
    \begin{picture}(\pw,\pht)(-\xi,-\yi)
     \multiput(0,200)(342,0){2}   {\line(5,3) {171}} % 7,8; 8a,1
     \multiput(171,303)(342,0){2} {\line(5,-3){171}} % 8,8a; 1,2
     \multiput(0,0)(342,0){3}     {\line(0,1) {200}} % 6,7;4a,8a
                                                     % 3,2
     \multiput(0,0)(342,0){2}     {\line(5,-3){171}} % 6,5; 4a,4
     \multiput(171,-103)(342,0){2}{\line(5,3) {171}} % 5,4a; 4,3
     \ifx#1Q
       \else\put(513,303)         {\line(0,1) {100}}  % sub. on 1
            \put(492,410)         {#1}    \fi
     \ifx#2Q
       \else\put(684,200)         {\line(5,3) {128}}  % sub. on 2
            \put(817,250)         {#2}    \fi
     \ifx#3Q
       \else\put(684,0)           {\line(5,-3){128}}  % sub. on 3
            \put(817,-100)        {#3}    \fi
     \ifx#4Q
       \else\put(513,-103)        {\line(0,-1){100}}  % sub. on 4
            \put(492,-283)        {#4}    \fi
     \ifx#5Q
       \else\put(171,-103)        {\line(0,-1){100}}  % sub. on 5
            \put(150,-283)        {#5}    \fi
     \ifx#6Q
       \else\put(0,0)             {\line(-5,-3){128}} % sub. on 6
            \put(-430,-116) {\makebox(300,87)[r]{#6}}   \fi  
     \ifx#7Q
       \else\put(0,200)           {\line(-5,3) {128}} % sub. on 7
            \put(-430,234)  {\makebox(300,87)[r]{#7}}   \fi
     \ifx#8Q
       \else\put(171,303)         {\line(0,1)  {100}} %sub. on 8
            \put(150,410)         {#8}    \fi
     \ifx#9S                                          %all single
       \else\put(316,174)         {\line(0,-1) {148}} %double 
                                                      %  4a,8a
            \put(162,-67)         {\line(-5,3) {126}} %double 5,6
            \put(36,191)          {\line(5,3)  {126}} %double 7,8
     \fi
     \ifx#9D\put(648,191)         {\line(-5,3) {126}} %double 2,1
            \put(520,-67)         {\line(5,3)  {126}} %double 4,3
     \fi
   \end{picture}       }                % end naphthalene macro
 \newcommand{\terpene}[9]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets the bicyclo(2.2.1)heptane ring         %
  % system with optional methyl groups at the one-carbon       %
  % bridge.                                                    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
 \begin{picture}(\pw,\pht)(-\xi,-\yi)
  \put(0,0)       {\line(5,1)  {196}}        % bond 5 to 4
  \put(196,39)    {\line(5,-2) {186}}        % bond 4 to 3
  \put(382,-35)   {\line(2,5)  {66}}         % bond 3 to 2
  \put(448,130)   {\line(-5,2) {186}}        % bond 2 to 1
  \put(262,204)   {\line(-5,-1){196}}        % bond 1 to 6
  \put(66,165)    {\line(-2,-5){66}}         % bond 6 to 5
  \put(196,39)    {\line(0,1)  {330}}        % long part of
                                             %  bridge
  \put(262,204)   {\line(-2,5) {66}}         % shorter part
                                             %  of bridge
  \ifx#1Q                                    % subst. on 1
    \else\put(262,204)   {\line(4,3)  {120}}
         \put(387,267)   {#1}            \fi
  \ifx#2Q                                    % subst. on 2
    \else\put(448,130)   {\line(4,3)  {120}}
         \put(573,193)   {#2}            \fi
  \ifx#3Q                                    % subst. on 3
    \else\put(382,-35)   {\line(5,-2) {120}}
         \put(507,-121)  {#3}            \fi
  \ifx#4Q                                    % subst. on 4
    \else\put(196,39)    {\line(2,-5) {56}}
         \put(231,-180)  {#4}            \fi
  \ifx#5Q                                    % subst. on 5
    \else\put(0,0)       {\line(-5,-2){139}}
         \put(-441,-95)  {\makebox(300,87)[r]{#5}}  \fi
  \ifx#6Q                                    % subst. on 6
    \else\put(66,165)    {\line(-4,3) {120}}
         \put(-362,216)  {\makebox(300,87)[r]{#6}}  \fi
  \ifx#7M\put(196,369)   {\line(4,3)  {120}} % methyl
         \put(196,369)   {\line(-4,3) {120}} %  groups
         \put(321,432)   {\small ${\rm CH_3}$}           
         \put(-226,425)                      %  on bridge
         {\makebox(300,87)[r]{\small ${\rm CH_3}$}} \fi
  \ifx#8Q\else
  \ifx#8O\put(443,142)   {\line(5,2)  {130}} % double-
         \put(453,118)   {\line(5,2)  {130}} %  bonded
         \put(583,155)   {$O$}               %  O on 2
    \else\put(448,130)   {\line(5,-2) {120}} % sec. subst.
         \put(573,44)    {#8}  \fi       \fi %  on 2
  \ifx#9Q\else
  \ifx#9D\put(368,-1)    {\line(2,5) {46}}   % double 3 to 2                  
    \else\put(382,-35)   {\line(4,3) {120}}  % second subst.
         \put(507,28)    {#9}    \fi     \fi %  on 3
 \end{picture}    }   % end terpene macro
 \newcommand{\steroid}[9]        {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets the steroid skeleton. Optional double  %
  % bonds and substituents make it possible to print the       %
  % structures of common steroids.                             %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
       \multiput(0,0)(342,0){3}    {\line(0,1) {200}} %3-2,
                                                      % 5-10,7-8
       \multiput(513,303)(342,0){3}{\line(0,1) {200}} %9-11,14-13,
                                                      %  15-16
       \multiput(0,200)(342,0){3}  {\line(5,3) {171}} %2-1,
                                                      % 10-9,
                                                      % 8-14
       \multiput(0,0)(342,0){2}    {\line(5,-3){171}} %3-4, 5-6
       \multiput(171,-103)(342,0){2}{\line(5,3) {171}} %4-5, 6-7
       \multiput(171,303)(342,0){2}{\line(5,-3){171}} %1-10, 9-8
       \multiput(513,503)(342,0){2}{\line(5,3) {171}} %11-12,
                                                      % 13-17
       \multiput(684,606)(342,0){2}{\line(5,-3){171}} %12-13,
                                                      % 17-16
       \put(855,303)               {\line(1,0) {342}} %14-15
       \put(855,503)               {\line(0,1) {128}} % methyl 18
       \put(795,638)               {\small ${\rm CH_3}$}
       \ifx#1D\put(36,191)         {\line(5,3)  {126}}% double
        \else\ifx#1Q                                  %  1 to 2
              \else\put(520,514)   {\line(-5,3)  {128}}
                   \put(506,492)   {\line(-5,3)  {128}}
                   \put(83,547)    {\makebox(300,87)[r]{#1}} \fi
       \fi                            % outside double & subst. 11  
       \ifx#2D\put(162,-67)        {\line(-5,3) {126}} % double 
        \else\ifx#2Q                                   %  4 to 3
              \else\put(-7,11)     {\line(-5,-3) {128}}
                   \put(7,-11)     {\line(-5,-3) {128}}
                   \put(-430,-116) {\makebox(300,87)[r]{#2}} \fi
       \fi                            % outside double & subst. 3
       \ifx#3Q
        \else\put(0,0)       {\line(-5,-3){128}}           % subst.         
             \put(-430,-116) {\makebox(300,87)[r]{#3}} \fi %  on 3
       \ifx#4D\put(178,-67)  {\line(5,3)  {126}}     \fi % double 
                                                         %  4 to 5
       \ifx#5D\put(378,9)    {\line(5,-3) {126}}         % double 
                                                         %  6 to 5
        \else\ifx#5Q
               \else\multiput(1011,606)(30,0){2} {\line(0,1) {100}}
                    \put(985,713)         {#5}         \fi
       \fi                             % outside double & subst. 17    
       \ifx#6D\put(316,174)  {\line(0,-1) {148}}     \fi % double 
                                                         % 5 to 10
       \ifx#6M\put(342,200)  {\line(0,1)  {128}}         % methyl 
                                                         %  19
              \put(282,335)  {\small ${\rm CH_3}$}     \fi
       \ifx#7Q
        \else\put(1026,606)  {\line(0,1)  {100}}         % lower  
                                                         %  subst.
             \put(995,713)   {#7}                    \fi %  part 
                                                         %  on 17
       \ifx#8Q
        \else\put(1026,791)  {\line(0,1)  {100}}         % upper 
                                                         %  subst.
             \put(995,900)   {#8}                    \fi %  part
                                                         %  on 17
       \ifx#9Q
        \else\put(1026,606)  {\line(1,0)  {128}}         % the other
             \put(1160,575)  {#9}                    \fi %  subst.
                                                         %  on 17
     \end{picture}       }                    % end steroid macro

 \newcommand{\hetthree}[8]       {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The hetthree macro draws a three-membered ring with one    %
  % hetero atom.                                               %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \begin{picture}(\pw,\pht)(-\xi,-\yi)
   \put(170,-170)  {#8}                        % hetero atom
   \put(0,0)       {C}                         % C-2
   \put(360,0)     {C}                         % C-3
   \put(80,30)     {\line(1,0)  {270}}         % bond 2-3
   \put(70,-10)    {\line(1,-1) {100}}         % bond 2-1
   \put(350,-10)   {\line(-1,-1){100}}         % bond 3-1
   \ifx#1Q                                     % substituent
     \else\put(210,-180) {\line(0,-1){80}}     %  on het. atom
          \put(180,-340) {#1}               \fi
   \ifx#6S\put(-10,30)   {\line(-1,0){140}}    % subst. on C-2
          \put(-460,-10) {\makebox(300,87)[r]{#2}} % with hor.
                                                   % bond
     \else\ifx#6H\put(-90,30)   {\line(-1,0) {140}}% bond and H
                 \put(-70,0)    {H}                %  on C-2
                 \put(-540,-10) {\makebox(300,87)[r]{#2}}
          \else  \put(-310,-10) {\makebox(300,87)[r]{#2}} \fi \fi
                                                   % no bond on 2
   \ifx#7S\put(440,30)   {\line(1,0) {140}}    % subst. on C-3
          \put(590,0)    {#3}                  %  with hor. bond
     \else\ifx#7H\put(430,0)    {H}            %  bond with H
                 \put(510,30)   {\line(1,0)  {140}}
                 \put(660,0)    {#3}
          \else  \put(445,0)    {#3}   \fi \fi % no bond on 3
   \ifx#4Q
     \else\put(40,80)    {\line(0,1) {140}}    % second subst.
          \put(-225,220) {\makebox(300,87)[r]{#4}} \fi % on C-2
   \ifx#5Q
     \else\put(400,80)   {\line(0,1) {140}}    % second subst.
          \put(360,230)  {#5}              \fi %  on C-3
  \end{picture}   }      % end hetthree macro
 \newcommand{\hetifive}[9]       {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The hetifive macro typesets a five-membered ring with one     %
  % hetero atom.                                                  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(342,0)          {\line(-5,-3) {140}}         % bond 2,1
    \put(342,0)          {\line(0,1)   {200}}         % bond 2,3
    \put(342,200)        {\line(-1,0)  {342}}         % bond 3,4
    \put(0,200)          {\line(0,-1)  {200}}         % bond 4,5
    \put(0,0)            {\line(5,-3)  {140}}         % bond 5,1
    \ifx#1Q
     \else\put(171,-137) {\line(0,-1)  {83}}          % subst.on 
          \put(135,-283) {#1}                     \fi % het.atom
    \ifx#2Q
     \else\ifx#2O\put(349,11) {\line(5,-3) {128}}     % outside
                 \put(335,-11){\line(5,-3) {128}}     %  double O
                 \put(475,-120)            {O}        %  on C-2
          \else\put(342,0)    {\line(5,-3) {128}}     % single
               \put(475,-100) {#2}                \fi %  subst.
    \fi                                               %  on C-2
    \ifx#3Q
     \else\put(342,200)  {\line(5,3)   {128}}         % subst. on
          \put(475,250)  {#3}                     \fi %  C-3
    \ifx#4Q
     \else\put(0,200)    {\line(-5,3)  {128}}         % subst. on
          \put(-430,234) {\makebox(300,87)[r]{#4}}\fi %  C-4
    \ifx#5Q
     \else\ifx#5O\put(-7,11)  {\line(-5,-3) {128}}    % outside
                 \put(7,-11)  {\line(-5,-3) {128}}    %  double O
                 \put(-200,-130)            {O}       %  on C-5
          \else\put(0,0)      {\line(-5,-3) {128}}    % single 
               \put(-430,-116){\makebox(300,87)[r]{#5}} \fi % sub.
    \fi                                               %  on C-5
    \ifx#6D\put(316,26)       {\line(0,1)  {148}} \fi % double 2,3
    \ifx#7D\put(316,174)      {\line(-1,0) {290}} \fi % double 3,4
    \ifx#8D\put(26,174)       {\line(0,-1) {148}} \fi % double 4,5
    \put(135,-130)            {#9}                    % hetero atom
  \end{picture}               }     % end one-hetero fivering macro
 \newcommand{\heticifive}[9]     {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The heticifive macro typesets a five-membered ring with     %
  % two hetero atoms separated by a carbon atom.                %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(342,0)          {\line(-5,-3) {140}}         % bond 2,1
    \put(342,0)          {\line(0,1)   {160}}         % bond 2,3
    \put(0,200)          {\line(1,0)   {300}}         % bond 4,3
    \put(0,200)          {\line(0,-1)  {200}}         % bond 4,5
    \put(0,0)            {\line(5,-3)  {140}}         % bond 5,1
    \ifx#1Q
     \else\put(171,-137) {\line(0,-1)  {83}}          % subst. on
          \put(135,-283) {#1}                     \fi %  het-1
    \ifx#2Q
     \else\ifx#2O\put(349,11)   {\line(5,-3) {128}}   % outside
                 \put(335,-11)  {\line(5,-3) {128}}   %  double O
                 \put(475,-120) {O}                   %  on C-2
          \else\put(342,0)      {\line(5,-3) {128}}   % single sub.
               \put(475,-100)   {#2}              \fi %  on C-2
    \fi
    \ifx#3Q
     \else\put(370,217)  {\line(5,3)    {100}}        % subst. on
          \put(475,250)  {#3}                     \fi %  on het-3
    \ifx#4Q
     \else\ifx#4O\put(-7,189)   {\line(-5,3) {128}}   % outside
                 \put(7,211)    {\line(-5,3) {128}}   %  double O
                 \put(-200,250) {O}                   %  on C-4
           \else\put(0,200)     {\line(-5,3) {128}}   % single sub.
                \put(-430,234)  {\makebox(300,87)[r]{#4}} \fi
    \fi                                               % on C-4
    \ifx#5Q
     \else\put(0,0)      {\line(-5,-3)  {128}}        % 1. single
          \put(-430,-116){\makebox(300,87)[r]{#5}}\fi %  subst. 
                                                      %  on C-5
    \ifx#6D\put(316,26)  {\line(0,1)    {130}}    \fi % double 2,3
    \ifx#7Q
     \else\ifx#7D\put(26,174)   {\line(0,-1) {148}}   % double 4,5
          \else\put(0,0)        {\line(-5,3) {128}}   % 2. subst.
               \put(-430,34)    {\makebox(300,87)[r]{#7}}  \fi
    \fi                                               %  on C-5
    \put(135,-130)              {#8}                  % het.atom 1
    \put(310,170)               {#9}                  % het.atom 3
   \end{picture}                }    % end heticifive macro
 \newcommand{\pyrazole}[8]      {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets the pyrazole ring with optional        %
  % substituents and double bonds inside and outside the       %
  % ring.                                                      %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(200,-84)        {\line(5,3)    {110}}        % bond 1,2
    \put(342,200)        {\line(0,-1)   {140}}        % bond 3,2
    \put(342,200)        {\line(-1,0)   {342}}        % bond 3,4
    \put(0,200)          {\line(0,-1)   {200}}        % bond 4,5
    \put(0,0)            {\line(5,-3)   {140}}        % bond 5,1
    \put(135,-130)       {N}                          % ring N-1
    \put(310,-30)        {N}                          % ring N-2 
    \ifx#1Q
     \else\put(171,-137) {\line(0,-1)   {83}}         % subst. on
          \put(150,-283) {#1}                     \fi %  on N-1
    \ifx#2Q
     \else\put(370,-17)  {\line(5,-3)   {100}}        % subst. on
          \put(475,-100) {#2}                     \fi %  N-2
    \ifx#3Q
     \else\ifx#3O\put(335,211)  {\line(5,3)  {128}}   % outside
                 \put(349,189)  {\line(5,3)  {128}}   %  double O
                 \put(475,250)  {O}                   %  on C-3
          \else\put(342,200)    {\line(5,3)  {128}}   % single sub.
               \put(475,250)    {#3}              \fi %  on C-3
    \fi
    \ifx#4Q
     \else\put(0,200)    {\line(-5,3)   {128}}        % single sub.
          \put(-430,234) {\makebox(300,87)[r]{#4}}\fi %  on C-4
    \ifx#5Q
     \else\ifx#5O\put(-7,11)    {\line(-5,-3){128}}   % outside
                 \put(7,-11)    {\line(-5,-3){128}}   %  double O
                 \put(-200,-130){O}                   %  on C-5
          \else\put(0,0)        {\line(-5,-3){128}}   % single sub.
               \put(-430,-116)  {\makebox(300,87)[r]{#5}}  \fi
    \fi                                               % on C-5
    \ifx#6D\put(316,174) {\line(0,-1)   {114}}    \fi % double 3,2
    \ifx#7D\put(316,174) {\line(-1,0)   {290}}    \fi % double 3,4
    \ifx#8D\put(26,174)  {\line(0,-1)   {148}}    \fi % double 4,5
  \end{picture}          }         % end pyrazole macro
 \newcommand{\hetisix}[9]       {              
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % The hetisix macro typesets a six-membered ring with        %
  % one hetero atom.                                           %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
    \begin{picture}(\pw,\pht)(-\xi,-\yi)
      \put(342,0)     {\line(-5,-3)  {140}}    % bond 2 to 1
      \put(0,0)       {\line(5,-3)   {140}}    % bond 6 to 1
      \put(342,0)     {\line(0,1)    {200}}    % bond 2 to 3
      \put(342,200)   {\line(-5,3)   {171}}    % bond 3 to 4
      \put(171,303)   {\line(-5,-3)  {171}}    % bond 4 to 5
      \put(0,200)     {\line(0,-1)   {200}}    % bond 5 to 6
      \ifx#7D                                   
        \put(316,26)  {\line(0,1)    {148}}    % double 2 to 3    
        \else\ifx#7Q
             \else\put(349,11)  {\line(5,-3){128}} % outside
                  \put(335,-11) {\line(5,-3){128}} %  double sub.
                  \put(475,-120){#7}         \fi   %  on C-2
      \fi
      \ifx#8D
        \put(36,191)  {\line(5,3)    {126}} \fi  % double 5 to 4
      \ifx#1D
        \put(36,9)     {\line(5,-3)  {110}}      % double 6 to 1
        \else\ifx#1Q
             \else\put(171,-220) {\line(0,1) {83}}
                  \put(150,-283) {#1}       \fi  % subst. on het.
      \fi
      \put(135,-130)  {#9}                       % the het.atom
      \ifx#2Q                                    
        \else\put(342,0)    {\line(5,-3)  {128}} % subst. on 2
             \put(475,-100)   {#2}
      \fi      
      \ifx#3Q
        \else\put(342,200)  {\line(5,3)   {128}} % subst. on 3
             \put(475,250)  {#3}
      \fi
      \ifx#4Q
        \else\put(171,303)  {\line(0,1)   {100}} % subst. on 4
             \put(150,410)  {#4}
      \fi
      \ifx#5Q
        \else\put(0,200)    {\line(-5,3)  {128}} % subst. on 5
             \put(-430,234) {\makebox(300,87)[r]{#5}}
      \fi
      \ifx#6Q
        \else\put(0,0)      {\line(-5,-3) {128}} % subst. on 6
             \put(-430,-116){\makebox(300,87)[r]{#6}}
      \fi                             % end sixring macro with
    \end{picture}     }               %  one hetero atom
  \newcommand{\pyrimidine}[9]        {          
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % This macro typesets the pyrimidine ring with optional      %
   % substituents and double bonds inside and outside the       %
   % ring.                                                      %
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
       \put(342,0)     {\line(-5,-3)  {140}}   % from 2 to 1
       \put(0,0)       {\line(5,-3)   {140}}   % from 6 to 1
       \put(342,0)     {\line(0,1)    {160}}   % from 2 to 3
       \put(171,303)   {\line(5,-3)   {140}}   % from 4 to 3
       \put(171,303)   {\line(-5,-3)  {171}}   % from 4 to 5
       \put(0,200)     {\line(0,-1)   {200}}   % from 5 to 6
       \put(135,-130)  {N}
       \put(310,170)   {N}
       \ifx#1Q
        \else\put(171,-137)  {\line(0,-1)  {83}} % sub. on N-1
             \put(150,-283)  {#1}               \fi
       \ifx#2Q
        \else\ifx#2O\put(349,11)  {\line(5,-3) {128}}  % outside
                    \put(335,-11) {\line(5,-3) {128}}  %  double O
                    \put(475,-120){O}                  %  on C-2
             \else\put(342,0)     {\line(5,-3) {128}}  % single
                  \put(475,-100)  {#2}           \fi   %  subst.
       \fi
       \ifx#3Q
        \else\put(370,217)   {\line(5,3)   {100}}      % subst.
             \put(475,250)   {#3}                \fi   %  on N-3
       \ifx#4Q
        \else\ifx#4O\put(158,303) {\line(0,1)  {100}}  % outside    
                    \put(184,303) {\line(0,1)  {100}}  %  double O
                    \put(130,410) {O}                  %  on C-4
             \else\put(171,303)   {\line(0,1)  {100}}  % single 
                  \put(150,410)    {#4}           \fi  %  subst.
       \fi                                             %  on C-4
       \ifx#5Q
        \else\put(0,200)     {\line(-5,3)   {128}}     % 1. subst.
             \put(-430,234)  {\makebox(300,87)[r]{#5}} \fi 
                                                       %  on C-5
       \ifx#6Q
        \else\ifx#6O\put(-7,11)   {\line(-5,-3){128}}  % outside
                    \put(7,-11)   {\line(-5,-3){128}}  %  double O
                    \put(-210,-130){O}                 %  on C-6
             \else\put(0,0)       {\line(-5,-3){128}}  % single s.
                  \put(-430,-116) {\makebox(300,87)[r]{#6}} \fi 
       \fi                                             %  on C-6
       \ifx#7D\put(306,9)    {\line(-5,-3)  {120}} \fi % 2,1 doub.
       \ifx#8D\put(180,267)  {\line(5,-3)   {120}}     % 4,3 doub.
        \else\ifx#8Q
             \else\put(0,200){\line(-5,-3)  {128}}     % 2. subst.
                  \put(-430,84) {\makebox(300,87)[r]{#8}}   \fi 
       \fi                                             %  on C-5
       \ifx#9D\put(26,174)   {\line(0,-1)   {148}} \fi % 5,6 doub.
   \end{picture}  }                     % end pyrimidine macro
 \newcommand{\pyranose}[9]   {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets monosaccharides with a pyran ring      %
  % system.                                                    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(588,0)         {\line(-1,-1) {159}}          % 1,2 bond
    \put(429,-159)      {\line(-1,0)  {270}}          % 2,3 bond
    \put(159,-159)      {\line(-1,1)  {159}}          % 3,4 bond
    \put(0,0)           {\line(1,1)   {159}}          % 4,5 bond
    \put(159,159)       {\line(1,0)   {225}}          % C-5 to O
    \put(394,130)       {\small O}                    % ring O
    \put(460,130)       {\line(1,-1)  {128}}          % O to C-1
    \ifx#1Q
     \else\put(588,0)   {\line(1,1)   {100}}          % beta sub.
          \put(700,75)  {#1}                     \fi  %  on C-1
    \ifx#2Q
     \else\put(588,0)   {\line(1,-1)  {100}}          % alpha sub.
          \put(700,-120){#2}                     \fi  %  on C-1
    \ifx#3Q
     \else\put(429,-159){\line(0,1)   {85}}           % up subst.
          \put(225,-75) {\makebox(250,87)[r]{#3}} \fi %  on C-2
    \ifx#4Q
     \else\put(429,-159){\line(0,-1)  {85}}           % down sub. 
          \put(400,-315){#4}                      \fi %  on C-2
    \ifx#5Q
     \else\put(159,-159){\line(0,1)   {85}}           % up subst. 
          \put(130,-73) {#5}                     \fi  %  on C-3
    \ifx#6Q
     \else\put(159,-159){\line(0,-1)  {85}}           % down sub.
          \put(130,-315){#6}                     \fi  %  on C-3              
    \ifx#7Q
     \else\put(0,0)     {\line(0,1)   {85}}           % up subst. 
          \put(-270,84) {\makebox(300,87)[r]{#7}} \fi %  on C-4
    \ifx#8Q
     \else\put(0,0)     {\line(0,-1)  {85}}           % down sub.
          \put(-270,-160){\makebox(300,87)[r]{#8}}\fi %  on C-4
    \put(159,159)       {\line(0,1)   {85}}           % C-6
    \put(130,250)       {\small ${\rm CH_{2}}$}       % sub. on
    \put(-370,245)      {\makebox(500,87)[r]{#9}}     %  C-6
  \end{picture}         }                 % end pyranose macro
 \newcommand{\furanose}[8]   {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets monosaccharides with a furan ring      %
  % system.                                                    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)
    \put(448,0)              {\line(-1,-2) {89}}      % bond 1,2
    \put(359,-179)           {\line(-1,0)  {270}}     % bond 2,3
    \put(89,-179)            {\line(-1,2)  {89}}      % bond 3,4
    \put(0,0)                {\line(5,3)   {188}}     % C-4 to O
    \put(192,110)            {\small O}               % ring O
    \put(260,113)            {\line(5,-3)  {188}}     % O to C-1
    \ifx#1Q
     \else\ifx#1N\put(448,0) {\line(0,1)   {380}}     % long bond 
                                                      %  for nucl.
          \else\put(448,0)   {\line(5,3)   {105}}     % beta sub.
               \put(558,50)  {#1}                 \fi %  on C-1
    \fi
    \ifx#2Q
     \else\put(448,0)        {\line(5,-3)  {105}}     % alpha sub.
          \put(558,-90)      {#2}                \fi  %   on C-1
    \ifx#3Q
     \else\put(359,-179)     {\line(0,1)   {85}}      % up subst.
          \put(155,-95)      {\makebox(250,87)[r]{#3}}\fi %on C-2
    \ifx#4Q
     \else\put(359,-179)     {\line(0,-1)  {85}}      % down sub.
          \put(330,-335)     {#4}                \fi  %  on C-2
    \ifx#5Q
     \else\put(89,-179)      {\line(0,1)   {85}}      % up sub.
          \put(60,-93)       {#5}                \fi  %  on C-3
    \ifx#6Q
     \else\put(89,-179)      {\line(0,-1)  {85}}      % down sub.
          \put(60,-335)      {#6}                \fi  %   on C-3
    \ifx#7Q
     \else\put(0,0)          {\line(0,-1)  {85}}      % down sub.
          \put(-270,-160)    {\makebox(300,87)[r]{#7}}\fi %on C-4
    \put(0,0)                {\line(0,1)   {85}}      % C-5
    \put(-30,90)             {\small ${\rm CH_{2}}$}
    \put(-530,80)            {\makebox(500,87)[r]{#8}}
  \end{picture}        }          % end furanose macro
 \newcommand{\purine}[9]           {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets the purine ring system with optional   %
  % double bonds and substituents.                             %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
    \begin{picture}(\pw,\pht)(-\xi,-\yi)
      \put(0,0)      {\line(0,1)   {160}}          % bond 2 to 1
      \put(0,0)      {\line(5,-3)  {140}}          % from 2 to 3
      \put(342,0)    {\line(-5,-3) {140}}          % from 4 to 3
      \put(342,0)    {\line(0,1)   {200}}          % from 4 to 5
      \put(316,174)  {\line(0,-1)  {148}}          % double 5 to 4
      \put(342,200)  {\line(-5,3)  {171}}          % from 5 to 6
      \put(171,303)  {\line(-5,-3) {140}}          % from 6 to 1
      \put(342,200)  {\line(1,0)   {300}}          % from 5 to 7
      \put(684,0)    {\line(0,1)   {160}}          % from 8 to 7
      \put(684,0)    {\line(-5,-3) {140}}          % from 8 to 9
      \put(342,0)    {\line(5,-3)  {140}}          % from 4 to 9
      \put(-32,170)  {\small N}                    % N at 1
      \put(135,-130) {\small N}                    % N at 3
      \put(652,170)  {\small N}                    % N at 7
      \put(477,-130) {\small N}                    % N at 9 
      \ifx#1Q
        \else\put(-128,277) {\line(5,-3) {100}}    % subst. on 1
             \put(-430,234) {\makebox(300,87)[r]{#1}}
      \fi
      \ifx#2D\put(36,9)     {\line(5,-3) {100}}    % double 2 to 3
        \else\put(-7,11)    {\line(-5,-3) {128}}
             \put(7,-11)    {\line(-5,-3) {128}}
             \put(-430,-116){\makebox(300,87)[r]{#2}}
      \fi                                          %outside double
                                                   %  bond on 2
      \ifx#3Q                                      % subst. on 3
        \else\put(171,-130) {\line(0,-1) {73}}
             \put(135,-283) {#3}
      \fi
      \ifx#4D\put(162,267)  {\line(-5,-3){110}} \fi % d. bond 6,1
      \ifx#5Q
        \else\multiput(158,303)(26,0){2} {\line(0,1) {100}}
             \put(135,410)  {#5}                % outside d.-bond
      \fi                                       % and subst. on 6
      \ifx#6Q                                   % single-bonded
        \else\put(171,303)  {\line(0,1)  {100}} % subst. on 6
             \put(150,410)  {#6}
      \fi
      \ifx#7Q                                   % subst. on 7
        \else\put(812,277)  {\line(-5,-3){100}}  
             \put(817,250)  {#7}
      \fi
      \ifx#8D\put(658,26)   {\line(0,1)  {125}} % d.-bond 8 to 7
        \else\put(691,11)   {\line(5,-3) {128}}
             \put(677,-11)  {\line(5,-3) {128}}
             \put(817,-110) {#8}                % outside d.-bond
      \fi                                       % and subst. on 8
      \ifx#9Q                                   % subst. on 9
        \else\put(513,-130) {\line(0,-1) {73}}
             \put(492,-283) {#9}
      \fi
      \end{picture}      }            % end purine macro

                   

        
  


 \newcommand{\fuseiv}[9]      {          
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a four-carbon fragment designed to     %
  % be connected to another ring at two places. As the         %
  % result, a sixring is fused linearly to another ring        %
  % system.                                                    %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)  
    \put(0,200)     {\line(5,3)  {171}}                % NE bond
    \put(171,303)   {\line(5,-3) {171}}                % SE bond
    \put(342,200)   {\line(0,-1) {200}}                % S  bond
    \put(342,0)     {\line(-5,-3){171}}                % SW bond
    \put(171,-103)  {\line(-5,3) {171}}                % NW bond
    \ifx#1Q
     \else\put(171,303)   {\line(0,1)   {100}}         % subst.
          \put(150,410)   {#1}                     \fi %  on top
    \ifx#2Q
     \else\put(342,200)   {\line(5,3)   {128}}         % subst. 
          \put(475,250)   {#2}                     \fi %  top rt.  
    \ifx#3Q
     \else\put(342,0)     {\line(5,-3)  {128}}         % subst.  
          \put(475,-100)  {#3}                     \fi %  low rt.
    \ifx#4Q
     \else\put(171,-103)  {\line(0,-1)  {100}}         % bottom
          \put(150,-283)  {#4}                     \fi %  subst.
    \ifx#5D \put(36,191)  {\line(5,3)   {126}}     \fi % NE double
    \ifx#6D \put(180,267) {\line(5,-3)  {126}}         % SE double
     \else\ifx#6Q
           \else\put(342,200)  {\line(5,-3)  {128}}    % 2. subst.
                \put(475,100)  {#6}                \fi %  top rt.
    \fi
    \ifx#7D \put(316,174) {\line(0,-1)  {148}}     \fi % S  double
    \ifx#8D \put(306,9)   {\line(-5,-3) {126}}         % SW double
     \else\ifx#8Q
           \else\put(342,0)    {\line(5,3)   {128}}    % 2. subst.
                \put(475,50)   {#8}                \fi % lower rt.
    \fi
    \ifx#9D \put(162,-67) {\line(-5,3)       {126}}\fi % NW double
  \end{picture}        }               % end fuseiv macro
 \newcommand{\fuseup}[9]   {          
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a four-carbon fragment designed to     %
  % connect to another ring at two places. As the result,      %
  % a sixring is fused angularly to the original ring.         %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi)  
    \put(-171,303)        {\line(0,1)   {200}}         % N  bond
    \put(-171,503)        {\line(5,3)   {171}}         % NE bond
    \put(0,606)           {\line(5,-3)  {171}}         % SE bond
    \put(171,503)         {\line(0,-1)  {200}}         % S  bond
    \put(171,303)         {\line(-5,-3) {171}}         % SW bond
    \ifx#1Q
     \else\put(-171,503)  {\line(-5,3)  {128}}      % upper left
          \put(-600,537)  {\makebox(300,87)[r]{#1}}\fi %  subst.
    \ifx#2Q
     \else\put(0,606)     {\line(0,1)   {100}}         % top sub.
          \put(-19,713)   {#2}                     \fi 
    \ifx#3Q
     \else\put(171,503)   {\line(5,3)   {128}}         % top rt.
          \put(304,553)   {#3}                     \fi %  subst.
    \ifx#4Q
     \else\put(171,303)   {\line(5,-3)  {128}}         % lower rt.
          \put(304,203)   {#4}                     \fi %  subst.
    \ifx#5D\put(-145,329) {\line(0,1)   {148}}     \fi % N double
    \ifx#6D\put(-135,494) {\line(5,3)   {126}}     \fi % NE double
    \ifx#7D\put(9,570)    {\line(5,-3)  {126}}     \fi % SE double
    \ifx#8D\put(145,477)  {\line(0,-1)  {148}}     \fi % S  double
    \ifx#9D\put(135,312)  {\line(-5,-3) {126}}     \fi % SW double
  \end{picture}      }                  % end fuseup macro
 \newcommand{\fuseiii}[6]    {          
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a three-carbon fragment designed to    %
  % be connected to another ring at two places. As the         %
  % result, a fivering is fused linearly to the original       %
  % ring system.                                               %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
   \begin{picture}(\pw,\pht)(-\xi,-\yi) 
    \put(0,200)     {\line(1,0)   {342}}               % E  bond
    \put(342,200)   {\line(0,-1)  {200}}               % S  bond
    \put(342,0)     {\line(-5,-3) {171}}               % SW bond
    \put(171,-103)  {\line(-5,3)  {171}}               % NW bond
    \ifx#1Q
     \else\put(342,200)   {\line(5,3)   {128}}         % upper rt.
          \put(475,250)   {#1}                     \fi %  subst.
    \ifx#2Q
     \else\put(342,0)     {\line(5,-3)  {128}}         % lower rt.
          \put(475,-100)  {#2}                     \fi %  subst.
    \ifx#3Q
     \else\put(171,-103)  {\line(0,-1)  {100}}         % bottom
          \put(150,-283)  {#3}                     \fi %  subst.
    \ifx#4Q
     \else\put(342,200)   {\line(5,-3)  {128}}         % 2. upper
          \put(475,100)   {#4}                     \fi %  rt. sub.
    \ifx#5Q
     \else\put(342,0)     {\line(5,3)   {128}}         % 2. lower
          \put(475,50)    {#5}                     \fi %  rt. sub.
    \ifx#6D \put(316,174) {\line(0,-1)  {148}}     \fi % S double
  \end{picture}      }                  % end fuseiii macro
 \newcommand{\cto}[3]   {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets an arrow for a chemical equation and   %
  % puts text above and below it.                              %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%        
  %
   \len=50   \multiply \len by #3                % calc. arrow
   \advance  \len by 120                         % length
     \begin{picture}(\pw,\pht)(-\xi,-\yi)
      \put(60,50)     {\vector(1,0)   {\len}}    % draw arrow
      \put(90,70)     {\makebox(\len,70)[l]
                      {\scriptsize ${\rm #1}$}}  % text on top
      \put(90,-40)    {\makebox(\len,70)[l]
                      {\scriptsize ${\rm #2}$}}  % text below
    \end{picture}     }      
 \newcommand{\sbond}[1]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a horizontal single bond of user-      %
  % specified length.                                          %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \xbox=#1  \advance \xbox by 2
  \hspace{1.5pt} \parbox{\xbox pt} {\rule{#1 pt}{0.4pt} }  
  \xbox=50     }  % end sbond macro
 \newcommand{\dbond}[2]    {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a horizontal double bond of user-     %
  % specified length.                                         %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \xbox=#1  \advance \xbox by 2
  \hspace{1.5pt}\parbox{\xbox pt} 
                       {\rule{#1 pt}{0.4pt}\vspace{-#2 pt}\\
                        \rule{#1 pt}{0.4pt}  }
  \xbox=50     }  % end dbond macro
 \newcommand{\tbond}[2]   {
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % This macro typesets a horizontal triple bond of user-     %
  % specified length.                                         %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %
  \xbox=#1   \advance  \xbox by 2
  \hspace{1.5pt} \parbox{\xbox pt} 
                        {\rule{#1 pt}{0.4pt}\vspace{-#2 pt}\\
                         \rule{#1 pt}{0.4pt}\vspace{-#2 pt}\\
                         \rule{#1 pt}{0.4pt}   }
  \xbox=50     }   % end tbond macro

